TorrentGuard: stopping scam and malware distribution in the BitTorrent ecosystem

In this paper we conduct a large scale measurement study in order to analyse the fake content publishing phenomenon in the BitTorrent Ecosystem. Our results reveal that fake content represents an important portion (35%) of those files shared in BitTorrent and just a few tens of users are responsible for 90% of this content. Furthermore, more than 99% of the analysed fake files are linked to either malware or scam websites. This creates a serious threat for the BitTorrent ecosystem. To address this issue, we present a new detection tool named TorrentGuard for the early detection of fake content. Based on our evaluation this tool may prevent the download of more than 35 millions of fake files per year. This could help to reduce the number of computer infections and scams suffered by BitTorrent users. TorrentGuard is already available and it can be accessed through both a webpage or a Vuze plugin.

==> program.tex <==
\section{Application}

Using the methodology described above we have implemented the system which continuously monitors the BitTorrent ecosystem. It leverage RSS feed of PirateBay to detect newly published torrents. Next, it tries to retrieve the IP of initial seeder. Moreover, it periodically monitors the webpages of the publishers in order to find these accounts which are removed by PirateBay. Among other data the system stores in a database following crucial information: IP addresses used to inject fake content and the list of fake torrents together with their hashes.

Finally we implement two publicly available\footnote{Access is granted to the parties by contacting the authors} ways of having access to our database. First, we have a web-based interface\footnote{faketorrentdetector.netcom.it.uc3m.es/Fake\_torrent/} where the user can upload the .torrent file to inspect. The system reads the hash of the content from .torrent file and by contacting the database it responds if the torrent contains malicious content. Secondly, we have implemented a plugin to the one of the most popular BitTorrent program Vuze\footnote{www.vuze.com}. This plugin is contacting our database each time the user wants to download new torrent. The hash of the torrent is send to our server which replies stating if the content is blacklisted or not. The goal of the application is to filter out fake publishers, improving downloaders experience and allowing them to avoid downloading fake content.
